Where to go next: Learning a Subgoal Recommendation Policy for Navigation Among Pedestrians

Robotic navigation in environments shared with other robots or humans remains challenging because the intentions of the surrounding agents are not directly observable and the environment conditions are continuously changing. Local trajectory optimization methods, such as model predictive control (MPC), can deal with those changes but require global guidance, which is not trivial to obtain in crowded scenarios. This paper proposes to learn, via deep Reinforcement Learning (RL), an interaction-aware policy that provides long-term guidance to the local planner. In particular, in simulations with cooperative and non-cooperative agents, we train a deep network to recommend a subgoal for the MPC planner. The recommended subgoal is expected to help the robot in making progress towards its goal and accounts for the expected interaction with other agents. Based on the recommended subgoal, the MPC planner then optimizes the inputs for the robot satisfying its kinodynamic and collision avoidance constraints. Our approach is shown to substantially improve the navigation performance in terms of number of collisions as compared to prior MPC frameworks, and in terms of both travel time and number of collisions compared to deep RL methods in cooperative, competitive and mixed multiagent scenarios.

==> sec/abstract.tex <==
\begin{abstract}

% This paper proposes a new framework for safe robot navigation among pedestrians, by introducing 

Robotic navigation through pedestrian environments remains challenging because the intentions of pedestrians are not directly observable and the environment conditions are continuously changing. 
Local trajectory optimization methods, such as model predictive control (MPC), can deal with those changes and provide guarantees but require global guidance, which is not trivial to obtain in crowded scenarios.
In this paper we propose to learn, via deep Reinforcement Learning (RL), an interaction-aware policy that provides longer term guidance to the local planner. In particular, in simulations with cooperative and non-cooperative agents, we train a deep network to recommend a subgoal for the MPC planner. The recommended subgoal is expected to help the robot in making progress towards its goal and accounts for the expected interaction with other agents. Based on the recommended subgoal, the MPC planner then optimizes the inputs for the robot satisfying its kinodynamic and collision avoidance constraints.
Our approach is shown to substantially improve the robot performance in terms of travel time and number of collisions as compared to prior MPC and deep RL methods in cooperative, competitive and mixed multiagent scenarios.

% Past works based on deep reinforcement learning methods work well in complex and dynamic environments with many agents. Nevertheless, such methods do not allow to define collision avoidance constraints explicitly. In contrast, optimization-based methods are highly efficient in generating trajectories handling constraints and vehicle dynamics but suffer from the curse of dimensionality. 
%Robot navigation among pedestrians in cluttered remains challenging, as motion planners must simultaneously satisfy vehicle dynamics and collision avoidance constraints while accounting for the interaction among them. In general, robot navigation systems are requested to generate motion plans leading the robot to reach a long-term goal position. However, to develop a complete plan to reach a long-term goal is not feasible because the pedestrian's intentions are not available, and the environment conditions are continually changing. This paper presents a sub-goal planning method that solves the problem of ``where" to go first to reach a long-term goal in cooperative and competitive scenarios.
%and thus, robots must continuously update their plans.
%As the pedestrian's intentions are not available to the robot and the environment conditions continously change, robots must update there plan
% This paper addresses the challenge of choosing a local subgoal
% Online optimization-based methods can handle the constraints, but their performance is hampered by a poor understanding of which ac
% Online optimization-based methods have been shown to generate trajectories

%Past works based on deep reinforcement learning methods have demonstrated to achieve state-of-the-art collision avoidance performance in complex and dynamic environments with a high number of agents. Nevertheless, such methods do not provide any collision avoidance guarantees and do not account for the agents' kynodynamic constraints. In contrast, optimization-based methods are highly efficient generating trajectories for an autonomous vehicle handling constraints and the vehicle dynamics but suffer from the curse of dimensionality.




\end{abstract}

==> sec/backup.tex <==
\subsection{SAC}
Soft Actor-Critic (SAC) is a off-policy algorithm proposed to reduce the number of training samples required to learn an optimal policy and ensure robust convergence during training to  change on the hyperparameters. During training, it not only optimizes the agent lifetime rewards but also it's policy entropy. High entropy means high exploration and low entropy high exploitation.

\begin{equation}
J(\pi)=\sum_{t=0}^{T} \mathbb{E}_{\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right) \sim \rho_{\pi}}\left[r\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right)+\alpha \mathcal{H}\left(\pi\left(\cdot | \mathbf{s}_{t}\right)\right)\right]
\end{equation}

where $\mathcal{H}$ is the entropy term weighted by $\alpha$.

SAC employs three function approximators (e.g. neural networks) to learn a value function $V_\psi(s_t)$, a soft Q-function $Q_\theta(S_T,A_T)$ and a policy function $\pi_\phi$, where ${\psi,\phi,\theta}$ are the model parameters. The usage of a separate value and Q function enhances the training convergence. 

The value function parameters are obtained by optimizing the following cost function:

\begin{equation}
J_{V}(\psi)=\mathbb{E}_{\mathbf{s}_{t} \sim \mathcal{D}}\left[\frac{1}{2}\left(V_{\psi}\left(\mathbf{s}_{t}\right)-\mathbb{E}_{\mathbf{a}_{t} \sim \pi_{\phi}}\left[Q_{\theta}\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right)-\log \pi_{\phi}\left(\mathbf{a}_{t} | \mathbf{s}_{t}\right)\right]\right)^{2}\right]
\end{equation}

The goal is to minimize the squared difference between the prediction of the value network and the expected prediction of the Q function plus the entropy of the policy function $\phi_\phi$ (measured here by the negative log of the policy function).

The Q-function parameters are obtained by optimizing the squared difference between the predicted Q value and a target value of a state/action tuple sample from the buffer replay. 

\begin{equation}
J_{Q}(\theta)=\mathbb{E}_{\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right) \sim \mathcal{D}}\left[\frac{1}{2}\left(Q_{\theta}\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right)-\hat{Q}\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right)\right)^{2}\right]
\end{equation}

where $\hat{Q}(\mathbf{s}_{t}, \mathbf{a}_{t})$ is:

\begin{equation}
\hat{Q}\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right)=r\left(\mathbf{s}_{t}, \mathbf{a}_{t}\right)+\gamma \mathbb{E}_{\mathbf{s}_{t+1} \sim p}\left[V_{\bar{\psi}}\left(\mathbf{s}_{t+1}\right)\right]
\end{equation}

For all (state, action) pairs in the experience replay buffer, we want to minimize the squared difference between the prediction of our Q function and the immediate (one time-step) reward plus the discounted expected Value of the next state, where $V_{\bar{\psi}}$ is the target value function.

We learn an optimal

\begin{equation}
J_{\pi}(\phi)=\mathbb{E}_{\mathbf{S}_{t} \sim \mathcal{D}}\left[D_{\mathrm{KL}}\left(\pi_{\phi}\left(\cdot | \mathbf{s}_{t}\right) \| \frac{\exp \left(Q_{\theta}\left(\mathbf{s}_{t}, \cdot\right)\right)}{Z_{\theta}\left(\mathbf{s}_{t}\right)}\right)\right]
\end{equation}

By employing the reparametrization trick we can express the objective function as follows:
\[
J_{\pi}(\phi)=\mathbb{E}_{\mathbf{s}_{t} \sim \mathcal{D}, \epsilon_{t} \sim \mathcal{N}}\left[\log \pi_{\phi}\left(f_{\phi}\left(\epsilon_{t} ; \mathbf{s}_{t}\right) | \mathbf{s}_{t}\right)-Q_{\theta}\left(\mathbf{s}_{t}, f_{\phi}\left(\epsilon_{t} ; \mathbf{s}_{t}\right)\right)\right]
\]



\begin{table*}[]
        \caption{Computation times of the proposed algorithm. \todo{Solver times on the left in bold and computation of collision free area on the right in [ms]}\LF{Can we write the total time (i.e., solver times and computation collision free area) and add between brackets the time needed for the computation of the collision free area? I would remove the min values to make it more compact}.}
        \centering
        \begin{tabular}{|l|llll|llll|llll|}
        \hline
        \multirow{2}{*}{\diagbox{Velocity [m/s]}{$T_{\textrm{horizon}}$ [s]}} & \multicolumn{4}{c|}{1}                                                                                                      & \multicolumn{4}{c|}{3}                                                                                                     & \multicolumn{4}{c|}{5}                                                                                                       \\ \cline{2-13} 
                                   & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Min.} & \multicolumn{1}{c}{Max.} & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Min.} & \multicolumn{1}{c}{Max.} & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Min.} & \multicolumn{1}{c}{Max.} & \multicolumn{1}{c|}{$\sigma$} \\ \hline
        1                  & \textbf{15} / 28                           & \textbf{1.5} / 1.9                       & \textbf{34.9} / 35.15                        & \textbf{6.7} / 32.5                               & \textbf{15} / 28                           & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                               & \textbf{15} / 28                           & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                               \\ \hline
        1.25            & \textbf{8.3} / 19.7                           & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                               & \textbf{15} / 28                           & \textbf{15} / 28                       &\textbf{15} / 28                         & \textbf{15} / 28                               & \textbf{15} / 28                           & \textbf{15} / 28                       & \textbf{15} / 28                        & \textbf{15} / 28                               \\ \hline
        1.5          & \textbf{7.2} / 16.9                              & \textbf{15} / 28                          & \textbf{15} / 28                            & \textbf{15} / 28                              & \textbf{15} / 28                          & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                                & \textbf{15} / 28                              & \textbf{15} / 28                          & \textbf{15} / 28                            & \textbf{15} / 28                                 \\ \hline
        \end{tabular}
        \label{tab:global_performance}
\end{table*}

\todo{Table~\ref{tab:global_performance} presents the results of the comparison with the baselines. Our proposed planner outperforms the.. }
\begin{table}[b]
        \caption{Statistics for the different motion planning strategies for static collision avoidance. MPCC: Model Predictive Contour Control; MPC: Tracking MPC; DW: Dynamic Window.}
        \centering
        \begin{tabular}{|p{1.34cm}|p{0.9cm}|p{0.54cm}|p{0.54cm}|p{0.54cm}|p{0.54cm}|p{1.12cm}|}
                \hline
                \multirow{2}{1.34cm}{Coordination strategies} & \multirow{2}{0.9cm}{Arrival time (s)} & \multicolumn{4}{c|}{Trajectory length (m)} & \multirow{2}{1.12cm}{Av.comp. time (ms)} \\ \cline{3-6}
                                                         &                                & min.      & max.     & av.      & std      &                                 \\ \hline
                MPCC                                       & 0.56                           & 4.82      & 7.09     & 5.72     & 0.89     & 15.2                               \\ \hline
                MPC                                       & 0.70                           & 4.31      & 4.54     & 4.43     & 0.09     & 115.3                               \\ \hline
                DW                                       & 0.70                              & 4.18         & 4.80        & 4.51        & 0.24        & 16.2                               \\ \hline
        \end{tabular}
        \label{tab:global_performance}
\end{table}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\# agents} & \multicolumn{3}{c|}{Clearance (m) (Mean / 99th percentile)} & \multicolumn{3}{c|}{\% failures (\% collisions / \% stuck)} & \multicolumn{3}{c|}{Traveled distance (m) (Mean / Std.)} \\ \hline
\multicolumn{2}{|c|}{}        & DW                & CADRL               & LMPCC               & DW               & CADRL               & LMPCC              & DW              & CADRL             & LMPCC             \\ \hline
\multicolumn{2}{|c|}{2}                &   1.10 / 0.63                &      0.75  / 0.63            &   0.97 / 0.65                  &  31.0 (30.0 / 1.0)                & 47.0 (45.0 / 3.0)                  &  \textbf{2.0 (0.0 / 2.0)  }                &    17.99  / 3.89           &     19.27 / 3.7              &     \textbf{15.8 / 3.23    }          \\ \hline
\multicolumn{2}{|c|}{4}                &        0.68 / 0.63           &      0.67/0.63                &     0.88 / 0.633                &  74.0 (71.0 / 3.0)                &  79.0 (76.0 / 3.0)                 &  \textbf{5.0 (2.0 / 3.0)  }                &     19.5 /5.28            &      21.34 / 4.4             &      \textbf{ 15.77 / 4.55 }           \\ \hline
\end{tabular}
 \label{tab:global_performance}
\end{table*}

==> sec/introduction.tex <==
%!TEX root=../main.tex

% The new proposed method links re-planning techniques on global scale with an optimization based controller approach on local scale to generate safe and smooth motion. Having both the ability of optimization-based planners that execute appropriate reactive behavior by explicitly incorporating constraints, as well as the efficiency and global convergence of search-based re-planning techniques, advantages of both methods are combined. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}


Autonomous robot navigation in crowds remains difficult due to the interaction effects among navigating agents.
Unlike multi-robot environments, robots operating among pedestrians require decentralized algorithms that can handle a mixture of other agents' behaviors without depending on explicit communication between agents.
% While pedestrians can safely navigate through these environments without explicit communication, decentralized and non-communicating methods for motion planning algorithms is necessary.

Several state-of-the-art collision avoidance methods employ model-predictive control (MPC) with online optimization to compute motion plans that respect important constraints \cite{paden2016survey}.
These constraints could include the vehicle's nonlinear kino-dynamics model or collision avoidance of static obstacles and other dynamic, decision-making agents (e.g., pedestrians).
Although online optimization becomes less computationally practical for extremely dense scenarios, modern solvers enable real-time motion planning in many situations of interest \cite{brito2019model}.

A key challenge is that the robot's global goal is often located far beyond the planning horizon, meaning that a local subgoal or cost-to-go heuristic must be specified instead.
This is straightforward in a static environment (e.g., using euclidean/diffusion~\cite{chen2016motion} distance), but the presence of pedestrians makes it difficult to quantify which subgoals will lead to the global goal quickest.
A body of work addresses this challenge with deep reinforcement learning (RL), in which agents learn a model of the long-term cost of actions in an offline training phase (usually in simulation) \cite{chen2017decentralized,chen2019crowd,everett2019collision,fan2020distributed}.
The learned model is fast-to-query during online execution, but the way learned costs/policies have been used to date does not provide guarantees on collision avoidance or feasibility with respect to the vehicle dynamics.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/animated_rl-mpc_5.png}
    \caption{Proposed navigation architecture. The subgoal planner observes the environment and suggests the next subgoal position to the local motion planner, the MPC. The MPC then computes a local trajectory and the robot executes the next optimal control command, which minimizes the distance to the provided position reference while respecting collision and kinodynamic constraints.}
    \label{fig:architecture_proposed}
\end{figure}

%In this paper, we introduce a Goal Oriented Model Predictive Control (GO-MPC) for navigation among cooperative and non-cooperative agents, as depicted in Fig~\ref{fig:architecture_proposed}. We employ RL to learn a policy providing an intermediate goal position to a MPC. Then, the MPC computes driving the 

In this paper, we introduce Goal Oriented Model Predictive Control (GO-MPC), which enhances state-of-art online optimization-based planners with a learned global guidance policy.
%This work enhances state-of-art online optimization-based planners with a learned global guidance policy.
In an offline RL training phase, an agent learns a policy that uses the current world configuration (vehicle and pedestrian states, global goal) to recommend a local subgoal for the MPC, as depicted in~\cref{fig:architecture_proposed}.
Then, the MPC generates control commands ensuring that the vehicle and collision avoidance constraints are satisfied while making progress towards the suggested subgoal.
Our approach maintains the kino-dynamic feasibility and collision avoidance guarantees inherent in an MPC formulation, while improving the average time-to-goal by leveraging past experience in crowded situations.

The main contributions of this work are:
\begin{itemize}
    %\item A trajectory optimization framework for motion planning in crowded environments that utilizes a learned cost for guidance and provides dynamic feasibility and collision avoidance guarantees;
    \item A goal-oriented Model Predictive Control method (GO-MPC) for navigation among interacting agents, which utilizes a learned global guidance policy (recommended subgoal) in the cost function and provides dynamic feasibility and collision avoidance guarantees;
    %\item An algorithm to train an RL agent whose actions are cascaded with an optimization-based controller.
    \item An algorithm to train an RL agent jointly with an optimization-based controller in mixed environments, which is directly applicable to real-hardware, reducing the sim to real gap.
    %\item leveraging the ability to learn from past experiences to improve navigation the cost-to-go or terminal constraint.
\end{itemize}

Finally, we present simulation results demonstrating an improvement over several state-of-art methods in challenging scenarios with realistic robot dynamics and a mixture of cooperative and non-cooperative neighboring agents. Our approach shows different navigation behaviors: navigating through the crowd when interacting with cooperative agents, avoiding congestion areas when non-cooperative agents are present and enabling communication-free decentralized multi-robot collision avoidance.

%We evaluate experiments show that our policy learn to behave different depending on the

%avoid congestion areas
%or more aggressive among cooperative agents

% Deep Reinforcement Learning (DRL) methods have achieve state-of-the-art collision avoidance performance in dynamic environments with a high number of agents \cite{fan2018fully}, \cite{everett2019collision}. Yet, such methods do not provide any collision avoidance guarantees and collision may happen if the surrounding agents policy differs from training environment. In addition, RL methods learn a reactive collision avoidance policy, and do not account for the kinodynamic constraints of the agents.

% However, in crowded environments the number locally optimal motion plans grows exponentially with the number of agents as well as the number of collision avoidance constraints needed to ensure safety. Hence, optimization-based methods suffer from the "curse of dimensionality" and do not scale environments with a high number of agents. Moreover, if the interaction is not take into account the even with perfect predictions optimization-based method fail to find a feasible solution due to the freezing robot problem \cite{trautman2010unfreezing}.

% a learned global guidance policy,  maintains safety guarantees while enabling agents to reach their goals more quickly. We propose to employ an RL agent learning a global guidance policy to a local optimization-based motion planner, a Model Predictive Controller (MPC). Then, the MPC generates control commands ensuring that the vehicles and collision avoidance constraints are satisfied. Our contributions are the following:

% \begin{itemize}
%     \item a joint training algorithm to learn a global guidance policy in scenarios with cooperative and non-cooperative agents
%     \item simulation and experimental results
% \end{itemize}

% Our results show:

% \begin{itemize}
%     \item faster training
%     \item combined framework allows achieved best collision avoidance performance
% \end{itemize}

\begin{comment}


Let's make sure we're on the same page in terms of what the potential contributions would be.
I think the problem formulation makes sense as a robotics person who wants robots to be able to accomplish that task, but from the perspective of solving a good research problem, it's most important we can point to that problem statement and say: this is what prior works have neglected and what we are solving.

Let's say the two most promising approaches in the recent literature are the RL and MPC strategies, what do those not handle properly or what's the tradeoff in using one vs. the other?

RL: doesn't consider the true vehicle dynamics, static obstacle collision checking is a bit ad-hoc also, ...

What's the key issue with the prior MPC approach we hope to address?
My understanding was: 
\begin{itemize}
\item the mpc sometimes gets stuck, unable to find a feasible soln. But what actually causes this?
\item where does the global reference path come from? If from A*/RRT/planner that ignores the dynamic objects, sure the MPC will go off-course to avoid the dynamic obstacles, but will still be trying to track a fundamentally flawed trajectory. So presumably, RL can generate a traj that's aware of dyanmic objects, meaning the MPC cost would be less impacted by trying to track a flawed traj, and really just impacted by the inability to account for veh dynamics?
\item the dynamic obstacle collision constraint/cost is only useful for the part of the planning horizon where the predictive model matches reality. in other words, if the horizon were 5sec but you only can really predict pedestrian motion for 0.2sec, then either we'd want a better predictive model or should ensure this uncertainty is this reflected in the cost/constraint
\end{itemize}

Does the MPC need to be tracking a nominal trajectory, or can the tracking stage cost be zero and terminal cost be relative to some sub-goal position, subject to dynamic/static collision constraints?

\end{comment}

==> sec/method_backup.tex <==
\section{METHOD}\label{sec:method}
% Clothoidal spline \cite{walton1990clothoidal}
The goal of the \ac{lmpcc} is to generate feasible and optimal motion with respect to the defined cost along the constructed local reference path. The \ac{lmpcc} framework contains the following contributions:
\begin{enumerate}
\item The use of a transition function between waypoints to eliminate the non-differentiable representation of the reference path (\cref{sec:reference_path}).
\item The application of a search routine to solve the approximation of the path progress estimation (\cref{sec:path_parameter}).
\item Static obstacle avoidance by explicitly constraining the control problem to an approximation of the collision-free area (\cref{sec:static_collision}).
\item A bound on the Minkowski sum of a circle and an ellipse for moving obstacles (\cref{sec:collision_avoidance2}).
\end{enumerate}
\subsection{Global planning / Generation of reference path}\label{sec:reference_path}
Given a goal position $\boldsymbol{p}_{\text{goal}}$, first, we use a global planning method (such as RRT \cite{kuffner2000rrt}) to compute a collision-free path through the static environment representation from an initial position $\boldsymbol{p}_0$. This global reference path $\pazocal{P}$ consists of $M$ points defined as $\boldsymbol{p}_m = [x^p_m,y^p_m] \in \W$ with $m \in \pazocal{M} := \{1,\dots,M\}$. Then, we split the path into segments delimited by $[x^p_m,y^p_m]$ and $[x^p_{m+1},y^p_{m+1}]$. We use cubic spline interpolation to obtain an analytical expression of the reference path for each segment, connecting each of the global reference path points with a polynomial of length $s_m$. The efficient implementation of \cite{tkspline} allows splines to be generated in $\order(q)$ and evaluation of the spline at a single point to be performed in $\order(\log (q))$, where $q$ is the number of input data points. This efficiency motivates our choice of local spline fitting during execution. Hence, we define the piece-wise spline segments as a function of the traveled distance along the reference path $\theta$. This path parameter equals zero at the start of each path segment and continuously increases along the segment. \cref{fig:mpcc_path} shows three reference path segments and the projected robot position on the reference path. 
\begin{figure}[t]
\centering
\includegraphics[trim={0cm 0 0cm 0cm},clip,width=0.8\columnwidth]{images/mpcc_path.pdf}
\caption{Reference path representation}
\label{fig:mpcc_path}
\end{figure}
Each path segment is composed of the interpolated reference trajectory points concatenated with a corresponding velocity reference, that is, $\boldsymbol{R}_m := [\boldsymbol{p}_m^{r^\textrm{T}},v_{\textrm{ref},m}]^\textrm{T}$. This velocity reference depends on the environment and should be provided by the route planning module. The cubic polynomials that define the local reference points $\boldsymbol{p}^r$ are a function of $\theta$ and are given by:
\begin{equation}\label{eq:analytic_reference_path}
\boldsymbol{p}^r_m(\theta)\! =\!
\begin{bmatrix}
x^r_m\\
y^r_m
\end{bmatrix}\! =\! \begin{bmatrix}
a^x_{m,1}\theta^3 + a^x_{m,2}\theta^2 + a^x_{m,3}\theta  + a^x_{m,4} \\
a^y_{m,1}\theta^3 + a^y_{m,2}\theta^2 + a^y_{m,3}\theta  + a^y_{m,4}
\end{bmatrix}
\end{equation}
where $[a^x_{m,1}, \dots, a^x_{m,4}]$ and $[a^y_{m,1},\dots, a^y_{m,4}]$ are the coefficients of the cubic polynomials at segment $m$ of both splines. \looseness=-1

We consider a limited set of path segments $\boldsymbol{R}_m \subset \pazocal{R}$ of the reference path. This allows to reduce the computational complexity of the planning problem and allows segments outside of the local reference path to change over time. We define the local reference path $\boldsymbol{L}^r$ at current time by linking $\eta$ path segments, starting from the $m$-th closest path segment, that is,
\begin{equation}\label{eq:L_m}
    \boldsymbol{L}^r = \{ R_i \in \pazocal{R} | i = [ m, \dots, m + \eta] \}
\end{equation}
%An analytical expression of the derivative of the local reference trajectory is given by
%\begin{align}
%\begin{split}
%\dot{x}^r_m = f_m^x(\theta)\sp{\prime} = 3a^x_1\theta^2 + 2a^x_2\theta + a^x_3\\
%\dot{y}^r_m = f_m^y(\theta)\sp{\prime}  = 3a^y_1\theta^2 + 2a^y_2\theta + a^y_3
%\end{split}
%\end{align}

\subsection{Selecting the number of path segments}
We provide a strategy to select $\eta$ to guarantee that the local reference path representation captures enough information of the global path to be tracked by the \ac{lmpcc}. In particular, we provide a strategy to select the length of the local reference path with respect to the prediction horizon. The number of path segments $\eta$ to be included in the local reference path is a function of the prediction horizon length, the individual path segment lengths, and the speed of the \ac{agv} at each time instance, as described below:
\begin{equation}\label{eq:eta}
\underbrace{\sum^{m + \eta}_{i = m} s_i}_{\text{Local reference path length}} \geq \underbrace{\tau \sum^{N}_{j = 0} v_{j}}_{\text{Traveled distance in horizon}}    ,
\end{equation}
where $\tau$ is the length of the discretization steps along the horizon.
We use an upper bound on~\eqref{eq:eta} by considering maximum longitudinal velocity $v_{\max}$ and select $\eta$ such that

% $\sum^{m + \eta}_{i = m} s_i \geq T_{\textrm{horizon}} \cdot v_{\max}$.

\begin{equation}\label{eq:eta_upper}
\sum^{m + \eta}_{i = m} s_i \geq T_{\textrm{horizon}} \cdot v_{\max}
\end{equation}
\subsection{Progress on reference path}\label{sec:path_parameter}
\ac{mpcc} keeps track of the path progress along the total reference path using the path parameter $\theta$. Finding the corresponding path parameter, however, involves solving another optimization problem which would increase the computational cost of the algorithm \cite{schwarting2017safe}. 
If the distance between waypoints is small in relation to their curvature, spline parametrization can be regarded as reasonable approximations of arc-length parametrizations. Therefore, conventional \ac{mpcc} assumes that the evolution of path parameter can be approximated by the traveled distance of the robot:
\begin{equation}\label{eq:path_variable}
\theta_{k+1} \approx \theta_k + v_k \tau
\end{equation}
where $v$ is the forward velocity of the controlled vehicle. The estimation of the path parameter, however, has shown to be quite coarse, especially when the AGV must deviate from the reference path during an avoidance maneuver. During such a maneuver, the path parameter starts drifting. \ac{lmpcc} resolves the problem of the drifting path parameter by performing line search around the estimated path parameter, as  Algorithm \ref{alg_theta} describes, resulting in the refined path variable estimation $\tilde{\theta}$. In particular, note that the evolution of the path variable in the prediction horizon still matches \cref{eq:path_variable}, while the initialization of the path parameter is done with the refined approximation $\tilde{\theta}_0$ at each iteration. 

\begin{algorithm}
\caption{Refined path variable estimation}\label{alg_theta}
\begin{algorithmic}[1]
\State {$\theta_0 = \theta_{previous} + v_k\tau$}
\State {$\text{window}= [\theta_0 - L_{\text{window}} : \theta_0 + L_{\text{window}}]$}
% \State $\textbf{int} \text{ N}_{\text{sample}}$
% \State $\textbf{double} \text{ window }$
\For {$\text{each } \theta_{\text{sample}} \text{ in window}$}
\State {$\text{Compute distance to } \theta_{\text{sample}}$}
\If {$\text{distance} < \text{distance}_{\text{min}}$}
\State {$\text{distance}_{\text{min}} = \text{distance}$}
\State {$\tilde{\theta}_0 = \theta_{\text{sample}}$}
\EndIf 
\EndFor
\end{algorithmic}
\end{algorithm}
\subsection{Maintaining continuity over the local reference path}
To concatenate the properties of separate reference path segments into the local reference path $\boldsymbol{L}^r$ that is tracked by the \ac{lmpcc}, we provide a differentiable expression of the corresponding parameters over the prediction horizon. We use a sigmoid activation function $\sigma$ to link $\eta$ path segments $\boldsymbol{R}_m$ as in \cref{eq:L_m}. In order to connect the analytical expressions of the reference path segments (\cref{eq:analytic_reference_path}), we multiply the piece-wise spline sections by their corresponding activation function $\sigma_m(\theta,s_m)$, as follows:
\begin{equation}\label{eq:concatenation}
    \bar{\boldsymbol{L}}^r(\theta) = \sum^{m+\eta}_{i = m} [   \bar{\boldsymbol{p}}^r(\theta_k)^\textrm{T}, \bar{v}_{ref}]^\textrm{T} \cdot \sigma_m(\theta,s_m)
\end{equation}
% \begin{align}\label{eq:concatenation}
% \begin{split}
%     L_k(\theta) &= \begin{bmatrix}
%     x^r(\theta)\\
%     y^r(\theta)\\
%     v^r(\theta)
%     \end{bmatrix} = \\
%     &= \sum^{m + \eta}_{i = m} \Bigg( \sigma_i(\theta,s_m) 
%     \cdot \prod_{j = m}^{i - 1}(1 - \sigma_i(\theta,s_m))
%     \begin{bmatrix}
%     x^r_i \\
%     y^r_i \\
%     v^r_i
%     \end{bmatrix}
%     \Bigg)
% \end{split}
% \end{align}

\subsection{Static Collision avoidance}\label{sec:static_collision_avoidance}
Figure \ref{fig:obstacles} provides and overview of our collision avoidance strategy that we discuss in more details below. The AGV is represented by $n_{\text{disc}}$ discs centered in $\boldsymbol{p}_j^B$, where $\boldsymbol{p}_j^B$ is the position on the $j$-th disc in the AGV body-frame and $n_{\textrm{disc}}$ is the number of discs used to bound the AGV, $j\in\pazocal{J}^{\textrm{disc}}:=\{1,2,\ldots,n_{\textrm{disc}}\}$.

\begin{figure}[h!]
\centering
\includegraphics[trim={0cm 0cm 0cm 7cm},clip ,width=\columnwidth]{images/polygon_vis.pdf}
\caption{Overview of our collision avoidance strategy.}
\label{fig:obstacles}
\end{figure}
%\subsubsection{Position constraints on static obstacles}\label{sec:static_collision}
It is assumed that the reference path is free of static obstacles. When the \ac{agv} deviates from the reference path, it should be guaranteed that static obstacles are avoided. Figure~\ref{fig:obstacles} shows how we approximate a collision-free region along the prediction horizon. In particular, we use the shifted optimal state sequence computed at the previous time instance $t-1$, namely, $\boldsymbol{z}^*_{1:N|t-1}$. Then, the $N$-th element to append to $\boldsymbol{z}^*_{1:N|t-1}$ is obtained by extrapolating from the last element of $\boldsymbol{z}^*_{1:N|t-1}$. The resulting vector is $\boldsymbol{\bar z}^*_{1:N|t-1}$. This sequence of states $\boldsymbol{\bar z}^*_{1:N|t-1}$ is used to center the circles depicted in Figure~\ref{fig:obstacles}. The collision-free region is then computed as follows. The radii are found by expanding each circle in the occupancy grid map of the environment until an occupied cell is detected. The radius of the collision free circle is denoted by $r_k$. The approximated collision free area is introduced as an inequality constraint on the current \ac{agv} position such that $\B(\boldsymbol{z}_k) \cup \pazocal{O}^{\textrm{static}} =\emptyset\,\forall\, k\in \{0,\dots,N\}$.

Given $\boldsymbol{\bar z}^*_{1:N|t-1}$, we enforce that the distance of the \ac{agv} with respect to these positions must be smaller than a circle with radius $\bar {r}_{k,j} := r_k - r_\textrm{disc} - \|\boldsymbol{p}_j^B\|_2^2$  $\forall k\in\{0,\dots,N\}$:
\begin{align}\label{eq:env_constraint}
\begin{split}
    c_{k}^{\textrm{env},j}\!(\boldsymbol{z}_k)\! = \bar {r}_{k,j} -  \|\boldsymbol{\bar p}^*_{k|t-1} - \boldsymbol{ p}_k\|_2^2 &\Big\rvert_{k,j} > 0
\end{split}
\end{align}

\subsection{Dynamic collision avoidance}\label{sec:dynamic_collision_avoidance}
Recall that each moving obstacle $A_i$ is represented by state $\boldsymbol{z}^{A_i}(t)$, and ellipse dimensions $a$ and $b$. The collision avoidance constraints can now be defined as an inequality constraint for each $j$-th disc bounding the robot with respect to the distance of each obstacle $i \in \{1,\dots,n\}$ at time k as depicted in \cref{fig:obstacles}. Omitting $i$ for simplicity, the inequality constraint on each disc of the \ac{agv} with respect to the obstacles is given by:
\begin{equation}\label{eq:ineq_constraint}
\begin{split}
\!\!\!c_k^{\textrm{obst},j}(\boldsymbol{z}_k) \!\!= \!\!\begin{bmatrix}
\Delta x_k^j\\
\Delta y_k^j
\end{bmatrix}^\textrm{T}\!\!\!\!
R(\psi)^\textrm{T}\!\!\begin{bmatrix}
\frac{1}{\alpha^2} & 0\\ 0 & \frac{1}{\beta^2}
\end{bmatrix}\!\! R(\psi)\!\!\!\ \begin{bmatrix}
\Delta x_k^j\\
\Delta y_k^j
\end{bmatrix}&\Bigg\rvert_{k,j} \!\!\!\!> 1
\end{split}
\end{equation}
The distance from disc $j$ to the obstacle is split into its $\Delta x^j$ and $\Delta y^j$ components as shown in \cref{fig:obstacles}. $R(\psi_k)$ is the rotation matrix corresponding to the heading of the obstacle and $\alpha$ and $\beta$ are the resulting axes of the ellipse constraint.

\begin{figure}[h!]
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip ,width=\columnwidth]{images/lambda.pdf}
\caption{Exact safety boundary computation}
\label{fig:bound}
\end{figure}

It is important to notice that previous approaches assumed that the Minkowski sum of an ellipse with a circle is an ellipsoid with semi-major $\alpha = a + r_{\text{disc}}$ and semi-minor axis $\beta = b + r_{\text{disc}}$ \cite{schwarting2017safe}. This assumption, however, is not correct and collision can still occur \cite{chen2017constrained} as represented in Fig. \ref{fig:bound} with the grey ellipsoid as the considered bound and in black the actual Minkowski sum. 
In this section we present what are the exact values for $\alpha$ and $\beta$ such that collision avoidance is guaranteed, represented by the orange ellipsoid.
% According with the theorem proposed by \cite{uteshev2015metric} the minimum distance between two quadratic shapes is the minimal positive zero of the polynomial:

\begin{lem}\label{eq:minimum_polynom}
        Let $X^TE_1X=1$ and $X^TE_2X=1$ be two quadratics in $\mathrm{R}^n$. Iff the matrix $E_1-E_{2}$ is sign definite then the square of the distance between the ellipsoid $X^TA_1X=1$ and the quadratic $X^TA_2X=1$ equals the minimal positive zero of the polynomial.
        \begin{align*}
                 F(z) = D_\lambda(\det{\lambda*E_1+(z-\lambda E_2)-\lambda(z-\lambda E_1E_2)})
        \end{align*}
        where $D$ stands for the discriminant of the polynomial treated w.r.t. $\lambda$ \cite{uteshev2015metric}.
\end{lem}

%We use a determinantal representation of the discriminant as defined in \cite{uteshev2015metric}. 
The minimum distance equation can be used to compute the minimum dimensions of an ellipsoid which correctly bounds the Minkowski Sum. Consider two ellipsoids $E_1= Diag(\frac{1}{(a)^2}\frac{1}{(b)^2})$ with semi-major axis $a$ and semi-minor axis $b$ and $E_2 = Diag(\frac{1}{(a+\delta)^2}, \frac{1}{(b+\delta)^2})$. $E_2$ representing the ellipsoid $E_1$  enlarged by $\delta$.
The \cref{eq:minimum_polynom} can now be used to obtain the minimum distance between $E_1$ and $E_2$ resulting in the following equation:

\begin{equation}
    Dist_{min}=\frac{4 a b \delta^2 + 2 a \delta^3 + 2 b \delta^3}{a^2 + 2 a b + b^2 + 2 a \delta + 2 b \delta}
\end{equation}

In order to find the correct bounding ellipsoid it is necessary to find the value of $\delta$ such that $Dist_{min} \ge r_{disc}$. Since the distance equals the minimal positive zero of the polynomials the solution can be found numerically in the positive neighborhood of zero. A close formula can also be obtained but due to its length it is not presented in this paper. The resulting bounding ellipse and shape of the Minkowski Sum can be observed in \cref{fig:bound}


In order to ensure collision-free motions the radius is enlarged by a factor $\lambda$: 
\begin{equation}
\begin{bmatrix}
\alpha\\
\beta
\end{bmatrix} = \begin{bmatrix}
a + \lambda r_{\text{disc}}\\
b + \lambda r_{\text{disc}}
\end{bmatrix}_{'}
\end{equation}
where $\lambda$ is computed such that the curvature of the constraint ellipsoid is a lower bound of the curvature of the Minkowski sum, as follows:
\begin{equation}\label{eq:new_bound}
    \lambda = \min\left[\begin{split}{\frac{(a^2 + b r)(1-\frac{2 a b}{a^2 + b r} + \sqrt{
   \frac{(a-2b)^2+b r)}{a^2 + b r})}}{2 b}}\\
   {\frac{(b^2 + a r)(1 -\frac{2 a b}{b^2 + a r} + \sqrt{\frac{(-2a+b)^2+a r}{b^2 + a r})}}{2 a}}
   \end{split}\right]
\end{equation}
This guarantees that the constraint ellipsoid entirely bounds the collision space.
% euqation for delta offset instead of lambda factor
%\begin{equation}\label{eq:new_bound}
    %\lambda = \min\left[\begin{split}{\frac{(a^2 + b r)(1-\frac{2 b(a+r)}{a^2 + %b r} + \sqrt{1+4
   %\frac{b^2-ab}{a^2 + b r})}}{2 b}}\\
   %{\frac{(b^2 + a r)(1 -\frac{2 a(b+r)}{b^2 + a r} + \sqrt{1+4\frac{b^2-a %b}{b^2 + ar})}}{2 a}}
%   \end{split}\right]
%\end{equation}
\subsubsection{Repulsion from dynamic obstacles}\label{sec:collision_avoidance3}
A penalty in the cost function that resembles repulsion from dynamic obstacles ensures clearance between the \ac{agv} and the obstacles. The penalty is defined as follows:
\begin{equation}\label{eq:repulsive}
J_{\text{repulsive}}(\boldsymbol{z}_k) = Q_R \sum^{n}_{i = 1} \bigg( \frac{1}{(\Delta x_k)^2 + (\Delta y_k)^2 + \gamma} \bigg) \quad \!,
\end{equation}
 where $Q_R$ is the weight on the repulsive forces \cite{Abbas2017}. The distance from the \ac{agv} to the dynamic obstacles is given in its separate $\Delta x_k$ and $\Delta y_k$ components as in \cref{fig:obstacles}. A small value $\gamma$ is introduced to avoid a division by zero, for numerical stability of the solver~\cite{Houska2011a}.
\subsection{Local Model Predictive Contouring Control} 
As introduced in \cref{sec:reference_path}, the global reference path $\pazocal{P}$ consists of $M$ segments, resulting in a local reference trajectory $\bar{\boldsymbol{L}}^r(\theta_k)$ with $\eta$ segments, starting from the $m$-th closest path segment. The local contour error $\epsilon^c$ and the longitudinal error $\epsilon^l$ are expressed as a function of $\theta$ as visualized in \cref{fig:mpcc}. 
\begin{figure}[t]
\centering
% \includegraphics[trim={11.5cm 0 1.8cm 14.5cm},clip,width=\columnwidth]{images/MPCC_robotframe.pdf}
\includegraphics[trim={11.5cm 0 1.8cm 14.5cm},clip,width=\columnwidth]{images/MPCC_worldframe.pdf}
\caption{Approximated contour and lag error on the path segment.}
\label{fig:mpcc}
\end{figure}
With $\bar{\boldsymbol{p}}^r(\theta_k)$ being the local reference path points, the contouring and longitudinal error vector $\boldsymbol{e}_k := [\tilde{\epsilon}^c(\boldsymbol{z}_k,\theta_k),\tilde{\epsilon}^l(\boldsymbol{z}_k,\theta_k)]^\textrm{T}$ is defined as follows:
\begin{align}
\boldsymbol{e}_k = 
\begin{bmatrix}
\sin \phi(\theta_k)& -\cos \phi(\theta_k)\\
- \cos \phi(\theta_k)&-\sin \phi(\theta_k)
\end{bmatrix}
\big( \boldsymbol{p}_k - \bar{\boldsymbol{p}}^r(\theta_k) \big).
\end{align}

% \begin{align}\label{eq:errors}
% \begin{split}
% \hat{\epsilon}^c(\boldsymbol{z}_k,\theta_k) &= \sin \phi(\theta_k) \big( x_k - x^r(\theta_k)\big) - \cos \phi(\theta_k) \big( y_k - y^r(\theta_k)\big)\\
% \hat{\epsilon}^l(\boldsymbol{z}_k,\theta_k) &= -\cos \phi(\theta_k) \big( x_k - x^r(\theta_k)\big) - \sin \phi(\theta_k) \big( y_k - y^r(\theta_k)\big)
% \end{split}
% \end{align}

%The path parameter allows the definition of two types of errors that can be included in the cost function to enforce that the \ac{agv} tracks the reference path. Ideally, the contour error, $\epsilon^c$, and the longitudinal error, $\epsilon^l$, would be expressed using the closest point to the local reference path as in \cref{fig:mpcc}.
In order to ensure progress along the reference path, the conventional MPCC scheme proposes to add a negative cost term proportional to the travelled distance. In contrast, we introduce a cost term that penalizes the deviation of the vehicle velocity $v_k$ with respect to a reference velocity $v_{\textrm{ref}}$. The reference velocity is provided according to \cref{eq:concatenation}, allowing the vehicle to adapt its speed according to the path segment that it is tracking. Now, the LMPCC tracking cost is defined as
$J_{\text{tracking}}(\boldsymbol{z}_k,\theta_k) = \boldsymbol{e}_k^TQ_{\epsilon}\boldsymbol{e}_k + Q_v(v_{ref} - v_k)^2$,
% where $Q_{\epsilon}$ and $Q_v$ are the weights on the path error and the reference velocity, respectively.
Additionally, the cost function also penalizes with weight $Q_u$ the inputs, that is, $J_{\text{input}}(\boldsymbol{z}_k,\theta_k) = \boldsymbol{u}_k^TQ_{u}\boldsymbol{u}_k$.
We can now formulate our \ac{lmpcc} control problem:
\begin{align}\label{eq:control_problem}
\begin{split}
J^* = &\min_{\boldsymbol{z}_{0:N},\boldsymbol{u}_{0:N-1}} \sum^{N-1}_{k =0} J(\mathbf z_k,\mathbf u_k, \theta_k) + J(\boldsymbol{z}_N,\theta_N) \\
\text{s.t.} \quad & \boldsymbol{z}_{k+1} := f(\boldsymbol{z}_{k},\boldsymbol{u}_{k}),  \\
& \theta_{k+1} = \theta_{k} + v_{k} \tau,  \\
& \boldsymbol{z}_{\min} \leq \boldsymbol{z}_k \leq \boldsymbol{z}_{\max},  \\
& \boldsymbol{u}_{\min} \leq \boldsymbol{u}_k \leq \boldsymbol{u}_{\max}, \\
& c_k^{\textrm{env}}(\boldsymbol{z}_k) > 0, \qquad \quad  \\
& c_k^{\textrm{obst},j}(\boldsymbol{z}_k) > 1, \quad \forall j,\, \forall \textrm{obst}\\
& \mathbf{z}_0 = z_{\textrm{init}}, \, \theta_0 = \tilde{\theta}  \\
\end{split}
\end{align}
where $ J(\mathbf z_k,\mathbf u_k, \theta_k): = J_{\text{tracking}}(\boldsymbol{z}_k,\theta_k)\! +\! J_{\text{repulsive}}(\boldsymbol{z}_k) \!+\! J_{\text{input}}(\boldsymbol{u}_k)$. \cref{alg_lmpcc} summarizes our design. Each control iteration, feedback steps are performed until either a \ac{kkt} condition \cite{kuhn1951} or the maximum number of iterations is satisfied (line ~\ref{alg:kkt}).

\begin{algorithm}
\caption{Local Model Predictive Control}\label{alg_lmpcc}
\begin{algorithmic}[1]
\State Given $z_0$, $z_{\textrm{goal}}$, $\pazocal{O}^{\textrm{static}}$, $\pazocal{O}_ k^{\textrm{dyn}}$, and $N$
\State {\textbf{Initialization}: $k = 0$}
    \State Build global path $\pazocal{P}$ \cref{eq:analytic_reference_path,eq:concatenation}
    \State Select $\eta$ according to \cref{eq:eta_upper}
    \State Build $\bar{\boldsymbol{L}}^r(\theta_k)$ according to  \cref{eq:analytic_reference_path,eq:concatenation}
\While{$\boldsymbol{z}_k \ne \boldsymbol{z}_{\textrm{goal}}$ in parallel}
    \State Process sensor data
    \State Estimate $\tilde{\theta}_0$ according to \cref{alg_theta}
    % \State Lock $\bar{\boldsymbol{L}}^r(\theta)$
    \State $\text{Compute }r_k \text{ along } \boldsymbol{\bar z}^*_{1:N|t-1}$
    \While{\texttt{iter} $< \textrm{\texttt{iter}}_{\max} \wedge \textrm{KKT} > \textrm{threshold}$} \label{alg:kkt}
            \State Solve \cref{eq:control_problem}
            \State $\texttt{iter}=\texttt{iter}+1$
    \EndWhile
    \State$\text{Apply } \boldsymbol{u^*_0}$
    \If{$\theta_k>s_k$}
        \State $k=k+1$
        \State Re-plan global path $\pazocal{P} \setminus \boldsymbol{p}^r$ 
        \State Build $\bar{\boldsymbol{L}}^r(\theta_k)$ according to  \cref{eq:analytic_reference_path,eq:concatenation}
    \EndIf 
\EndWhile
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
% \caption{Local Model Predictive Control}\label{alg_lmpcc}
% \begin{algorithmic}[1]
% \State Given $z_0$, $z_{\textrm{goal}}$, $\pazocal{O}^{\textrm{static}}$, $\pazocal{O}_ k^{\textrm{dyn}}$, and $N$
% \State {\textbf{Initialization}: $k = 0$}
%     \State Build global path $\pazocal{P}$
%         \For{$m = 0,1,2, \ldots M-1$}
%             \State Build $\boldsymbol{R}_m$ according to \cref{eq:analytic_reference_path}
%         \EndFor 
%     \State Select $\eta$ according to \cref{eq:eta_upper}
% \While{$\boldsymbol{z}_k \ne \boldsymbol{z}_{\textrm{goal}}$ in parallel}
%     \State Process sensor data
%     \State Estimate $\tilde{\theta}_0$ according to \cref{alg_theta}
%     \State Lock $\bar{\boldsymbol{L}}^r(\theta)$
%     \For{$m \ne k \in $range($M$)}
%         \State Re-plan global path: $\boldsymbol{R}_m$ 
%         \State Build $\overline{R}$: polynomial fitting: $\boldsymbol{R}_m$
%     \EndFor 
%     \State $\text{Compute }r_k \text{ along } \boldsymbol{\bar z}^*_{1:N|t-1}$
%     \While{\texttt{iter} $< \textrm{\texttt{iter}}_{\max} \wedge \textrm{KKT} > \textrm{threshold}$}
%             \State Solve \cref{eq:control_problem}
%             \State $\texttt{iter}=\texttt{iter}+1$
%     \EndWhile
%     \State$\text{Apply } \boldsymbol{u^*_0}$
%     \If{$\theta_k>s_k$}
%         \State $k=k+1$
%     \EndIf 
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

==> sec/results.tex <==
\section{RESULTS}\label{sec:results} 

This section quantifies the performance throughout the training procedure, provides an ablation study, and compares the proposed method (sample trajectories and numerically) against two baseline approaches:
\begin{itemize}
    \item MPC: Model Predictive Controller from \cref{sec:lmpcc} with final goal position as position reference, $\vp_{\textrm{ref}}=\vg$
    \item DRL~\cite{everett2019collision}:  state-of-the-art Deep Reinforcement Learning approach for multi-agent collision avoidance
\end{itemize}
Experiments use second-order robot dynamics and consider environments with cooperative and non-cooperative agents to represent realistic robot/pedestrian behavior.
Animations of sample trajectories accompany the paper.

\subsection{Experimental setup}\label{sec:experiment_setup}
%We implemented the described policy network architecture using TensorFlow \cite{abadi2016tensorflow}.
The proposed training algorithm builds upon the open-source PPO implementation provided in the Stable-Baselines \cite{stable-baselines} package. We used a laptop with an Intel Core i7 and 32~GB of RAM for training. To solve the non-linear and non-convex MPC problem of \cref{eq:control_problem}, we used the ForcesPro~\cite{FORCESPro} solver. If no feasible solution is found within the maximum number of iterations, then the ego-agent decelerates. Also, all MPC methods used in this work consider collision constraints on only the closest six agents so that the optimization problem can be solved in less than 20ms. Hyperparameter values are summarized in \cref{tab:hyperparameters}.

%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}|}
\begin{table}[t]
\caption{Hyper-parameters. }
\label{tab:hyperparameters}
\centering
\begin{tabular}{|p{0.4\columnwidth}|P{0.2\columnwidth}|}
\hline
Planning Horizon $H$ & 2 s  \\ \hline
Number of Stages & 20 \\ \hline
$\gamma$ & 0.99 \\ \hline
Clip factor & 0.1 \\ \hline
Number of mini batches & 2048 \\ \hline
Learning rate & $10^{-4}$ \\ \hline
$r_{\textrm{goal}}$ & 3 \\ \hline
$r_{\textrm{collision}}$ & -10 \\ \hline
\end{tabular}
\end{table}

\subsection{Training procedure}\label{sec:training}
Each training episode consists of a random number of agents and a random scenario from the following categories:
\begin{itemize}
    \item \textbf{Symmetric swapping}: Each agent's position is randomly initialized in different quadrants of the $\mathbb{R}^2$ x-y plane, where all agents have the same distance to the origin. Each agent's goal is to swap positions with an agent from the opposite quadrant.
    \item \textbf{Asymmetric swapping}: As before, but all agents are located at different distances to the origin.
    %\item Each agent is assigned a position on a virtual circle centered on the plane $\mathbb{R}^2$. We sample a random circle radius $r_{\textrm{Circle}}$, , then for each pair of agents we randomly sample an angle $\psi\in [0,2\pi]$ and 
    \item \textbf{Pair-wise swapping}: Random initial positions; pairs of agents' goals are each other's intial positions
    \item \textbf{Random}: Random initial \& goal positions
\end{itemize}

At the start of each episode, each non-ego-agent's policy is sampled from a binomial distribution (80\% cooperative, 20\% non-cooperative). Moreover, for the cooperative agents we randomly sample a cooperation coefficient $c^i \sim \pazocal{U}(0.1,1)$.
\cref{fig:coll_evol_training} shows the evolution of the ego-agent average reward and the percentage of failure episodes. 
The top sub-plot compares our method average reward with the two baseline methods: DRL~\cite{everett2019collision} (with pre-trained weights) and MPC. The average reward for the baseline methods (orange, yellow) drops as the number of agents increases (each vertical bar). In contrast, our method (blue) improves with training and eventually achieves higher average reward for 10-agent scenarios than baseline methods achieve for 2-agent scenarios. The bottom plot demonstrates that the percentage of collisions decreases throughout training despite the number of agents increasing.
%\meXX{Remove when you remove the bottom plot? $\Rightarrow$ The bottom sub-plot shows the number of successful episodes per rollout. As the number of agents increases, the number of successful events also decreases because the scenarios are more complex, requiring more steps to reach the goal. Nevertheless, around 10 million training steps, the number of successful events continuously increases while the number of collisions keeps going down, demonstrating that our method's performance keeps improving.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/training_curves_new_reduced.pdf}
    \caption{Moving average rewards and percentage of failure episodes during training. The top plot shows our method average episode reward vs DRL~\cite{everett2019collision} and simple MPC.}
    \label{fig:coll_evol_training}
\end{figure}

\subsection{Ablation Study}\label{sec:reward}
A key design choice in RL is the reward function; here, we study the impact on policy performance of three variants of reward. The \textit{sparse} reward uses $r_t=0$ (only non-zero reward upon reaching goal/colliding). The \textit{time} reward uses $r_t=-0.01$ (penalize every step until reaching goal). The \textit{progress} reward uses $r_t = 0.01*(\norm{\vs_t-\vg}-\norm{\vs_{t+1}-\vg})$ (encourage motion toward goal). Aggregated results in Table \ref{tab:reward_performance} show that the resulting policy trained with a time reward function allows the ego-agent to reach the goal with minimum time, to travel the smallest distance, and achieve the lowest percentage of failure cases. Based on these results, we selected the policy trained with the time reward function for the following experiments.
%All experiments use the values $r_{\textrm{goal}}=3$ and $r_{\textrm{collision}}=-10$ for \cref{eq:reward}.
%\meXX{do these go in table 1 instead? what about $r_t$?}\BF{$r_t$ was previously defined in the text.}

%\BF{Secondly, we compared the training performance with and without collision constraints. The results show that having collision avoidance constraints during training increases significantly the training speed and policy performance. (This is still to be finished.)}

\begin{table*}[]
 \caption{Ablation Study: Discrete reward function leads to better policy than sparse, dense reward functions. Results are aggregated over 200 random scenarios with $n \in \{6,8,10\}$ agents. %\meXX{Better than sparse/dense/discrete would be sparse/time penalty/progress penalty?}
 }
        \centering
\begin{tabular}{|p{2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|}
\hline
\multicolumn{2}{|c|}{} & \multicolumn{3}{c|}{Time to Goal [s]} & \multicolumn{3}{c|}{\% failures (\% collisions / \% timeout) } & \multicolumn{3}{c|}{Traveled distance Mean [m]} \\ \hline
\multicolumn{2}{|c|}{\# agents}                    & \multicolumn{1}{c|}{6}                & \multicolumn{1}{c|}{8}       & \multicolumn{1}{c|}{10}                        & \multicolumn{1}{c|}{6}                &\multicolumn{1}{c|}{8}     & \multicolumn{1}{c|}{10}                       & \multicolumn{1}{c|}{6}                & \multicolumn{1}{c|}{8}       &\multicolumn{1}{c|}{10}        \\  \hline \hline
\multicolumn{2}{|l|}{Sparse Reward}                            & \multicolumn{1}{c|}{8.00}      &  \multicolumn{1}{c|}{8.51}          &     \multicolumn{1}{c|}{ 8.52}          & \multicolumn{1}{c|}{0 (0 / 0)}       & \multicolumn{1}{c|}{ 1 (0 / 1)}     &   \multicolumn{1}{c|}{2 (1 / 1) }            &  \multicolumn{1}{c|}{ 13.90}                &   \multicolumn{1}{c|}{14.34}       & \multicolumn{1}{c|}{14.31}   \\ \hline
\multicolumn{2}{|l|}{Progress Reward}                      &  \multicolumn{1}{c|}{8.9}     &  \multicolumn{1}{c|}{8.79}       &    \multicolumn{1}{c|}{9.01 }         & \multicolumn{1}{c|}{ 2 (1 / 1)}    &  \multicolumn{1}{c|}{3 (3 / 0)}        &  \multicolumn{1}{c|}{1 (1 / 0)  }        &  \multicolumn{1}{c|}{14.75}   &   \multicolumn{1}{c|}{14.57}       & \multicolumn{1}{c|}{14.63}    \\ \hline
\multicolumn{2}{|l|}{Time Reward}                &   \multicolumn{1}{c|}{\textbf{7.69}}              &   \multicolumn{1}{c|}{\textbf{8.03}}            &  \multicolumn{1}{c|}{\textbf{8.12}}       & \multicolumn{1}{c|}{\textbf{  0 (0 / 0) }}    &  \multicolumn{1}{c|}{\textbf{0 (0 / 0)   }}        & \multicolumn{1}{c|}{\textbf{   0 (0 / 0)   }}      & \multicolumn{1}{c|}{\textbf{13.25}}                &\multicolumn{1}{c|}{\textbf{14.01} }    &      \multicolumn{1}{c|}{\textbf{14.06}}         \\ 
\hline
\end{tabular}
 \label{tab:reward_performance}
\end{table*}

\subsection{Qualitative Analysis}

This section compares and analyzes trajectories for different scenarios. \cref{fig:2_agents_swap} shows that our method resolves a failure mode of both RL and MPC baselines.
The ego-agent has to swap position with a non-cooperative agent (red, moving right-to-left) and avoid a collision. We overlap the trajectories (moving left-to-right) performed by the ego-agent following our method (blue) versus the baseline policies (orange, magenta). The MPC policy (orange) causes a collision due to the dynamic constraints and limited planning horizon. The DRL~\cite{everett2019collision} policy avoids the non-cooperative agent, but due to its reactive nature, only avoids the non-cooperative agent when very close, resulting in larger travel time. Finally, when using our approach, the ego-agent initiates a collision avoidance maneuver early enough to lead to a smooth trajectory and faster arrival at the goal.

\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{images/swap2_cropped.pdf}
	\caption{Two agents swapping scenario. In blue is depicted the trajectory of ego-agent, in red the non-cooperative agent, in purple the GA3C agent and, in orange the MPC.}
	\label{fig:2_agents_swap}
\end{figure}

\begin{figure}

    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
    	\includegraphics[width=\textwidth, trim = 0 0 0 0, clip]{images/012_MPC_6agents.pdf}
    	\captionsetup{justification=centering}
    	\caption{GO-MPC with 5 agents \\ (all coop.)}
    	\label{fig:mix_agents_cooperative}
    \end{subfigure}%
    %\vspace{1mm}
    \hspace{1mm}
    \begin{subfigure}{0.48\linewidth}
        \centering
    	\includegraphics[width=\textwidth, trim = 0 0 0 0, clip]{images/011_MPC_8agents.pdf}
    	\captionsetup{justification=centering}
    	\caption{GO-MPC with 7 agents \\ (2 coop., 5 non-coop.)}
    	\label{fig:mix_agents_mix}
    \end{subfigure}%
    \caption{Sample trajectories with mixed agent policies (ego-agent: blue, cooperative: green, non-cooperative: red). The GO-MPC agent avoids non-cooperative agents differently than cooperative agents.}
    \label{fig:mix_agents}
\end{figure}

\begin{figure}

    \centering
    \begin{subfigure}{0.31\linewidth}
        \centering
    	\includegraphics[width=\textwidth, trim = 0 0 0 0, clip]{images/V1_2.pdf}
    	\caption{DRL \cite{everett2019collision}.}
    	\label{fig:homo_agents_rl}
    \end{subfigure}%
    \hspace{1mm}
    \begin{subfigure}{0.31\linewidth}
        \centering
    	\includegraphics[width=\textwidth, trim = 0 0 0 0, clip]{images/v2.pdf}
    	\caption{DRL-2.}
    	\label{fig:homo_agents_rl_d2}
    \end{subfigure}%
    \hspace{1mm}
    \begin{subfigure}{0.31\linewidth}
        \centering
    	\includegraphics[width=\textwidth, trim = 0 0 0 0, clip]{images/000_MPCRLPolicy_8agents.png}
    	\caption{GO-MPC.}
   	\label{fig:homo_agents_mpcrl}
    \end{subfigure}%
    \caption{Trajectories for 8 agents swapping positions. To simulate a multi-robot environment, all agents follow the same policy.}
    \label{fig:homo_agents}
\end{figure}

%\begin{figure*}[!t]
%  \centering
%  \begin{minipage}{\textwidth}
%    \includegraphics[height=5cm,width=17.8cm,trim={0cm 0cm 0cm 0cm},clip]{images/mixed_scenarios.png} % scene5_step_11
%    \caption*{\textit{a)} This sub-figure illustrates three sample results obtained for the asymmetric swapping scenario with mixed-agents, cooperative and non-cooperative. Green depicts the cooperative agents, red the non-cooperative and blue the ego-agent.}
%    \label{fig:mix_agents1} 
%  \end{minipage}
%   \vspace{1mm}

%    \begin{minipage}{\textwidth}
%      \includegraphics[height=5cm,width=17.8cm,trim={0cm 0cm 0cm 0cm},clip]{images/homogeneous_scenarios.png} %scene12_step_22 scene12_step_20 is a good one 13_8 too
%      \caption*{\textit{b)}  Three examples of the asymmetric swapping scenario where all the agents following our navigation policy. Each agent is assigned a different color. The goal position is depicted with a star symbol of the agent's color.}
%      \label{fig:homo_agents1}
%    \end{minipage}
%    \hspace{10mm}
%  \caption{ \BF{Split in two images. add also the analysis path among cooperative vs safe path among non cooperative}Simulation results for the asymmetric swapping scenario with mixed and homogeneous agents and,  for $n \in \{6,8,10\}$ agents.
%  \meXX{Let's replace 1 of the bottom right 2 examples to be one where the MPC-RL agents go more straight to their goals.}
%  }
%  \label{fig:qualitative_results}
%\end{figure*}   

We present results for mixed settings in \cref{fig:mix_agents} and homogeneous settings in \cref{fig:homo_agents} with $n \in \{6,8,10\}$ agents. In mixed settings, the ego-agent follows our proposed policy while the other agents either follow an RVO \cite{van2008reciprocal} or a non-cooperative policy (same distribution as in training). \cref{fig:mix_agents} demonstrates that our navigation policy behaves differently when dealing with only cooperative agents or both cooperative and non-cooperative. Whereas in \cref{fig:mix_agents_cooperative} the ego-agent navigates through the crowd, \cref{fig:mix_agents_mix} shows that the ego-agent takes a longer path to avoid the congestion in the middle.

In the homogeneous setting, all agents follow our proposed policy.
\cref{fig:homo_agents} shows that our method achieves faster time-to-goal than two DRL baselines. Note that this scenario was never introduced during the training phase, nor have the agents ever experienced other agents with the same policy before. Following the DRL policy~\cite{everett2019collision} (\cref{fig:homo_agents_rl}), all agents navigate straight to their goal positions leading to congestion in the center with reactive avoidance. The trajectories from the DRL-2 approach (\cref{fig:homo_agents_rl_d2}) are more conservative, due to the limited acceleration available. In contrast, the trajectories generated by our approach (\cref{fig:homo_agents_mpcrl}), present a balance between going straight to the goal and avoiding congestion in the center, allowing the agents to reach their goals faster and with smaller distance traveled.

\subsection{Performance Results}\label{sec:results_dynamic}

This section aggregates performance of the various methods across 200 random scenarios.
Performance is quantified by average time to reach the goal position, percentage of episodes that end in failures (either collision or timeout), and the average distance traveled.
To analyze the impact of a realistic dynamics model for the ego-agent, we consider two variants of the DRL~\cite{everett2019collision} method: the same algorithm was used to train an agent with a first-order dynamics model, DRL~\cite{everett2019collision}, and a second-order dynamics model, DRL-2~\cite{everett2019collision}. All methods are evaluated with second-order dynamics.
%Furthermore, to evaluate the guidance policy, we compare our method, GO-MPC, with a variant without collision avoidance constraints on, the GO-MPC-Off.

The numerical results are summarized in \cref{tab:global_performance}. Our method outperforms all baselines on the collision avoidance performance for both mixed agents and homogeneous scenarios. Although MPC has the minimum average time to goal and traveled distance for the mixed agent's scenario, its collision avoidance performance is poor. Moreover, for the homogeneous scenario, MPC is unperformed by all methods in all metrics.
For the homogeneous scenario, our approach is more conservative than the DRL~\cite{everett2019collision} and MPC baselines resulting in a larger average traveled distance.
Nevertheless, our method is more time-efficient than all baselines and less conservative than the DRL-2~\cite{everett2019collision} method achieving a lower average travel distance.% in terms of traveled distance, and achieves the minimum average time to goal 


Finally, considering higher-order dynamics when training the DRL~\cite{everett2019collision} agents (DRL-2) allows improving the collision avoidance performance. However, it also increases the average time to goal and traveled distance, meaning a more conservative policy that still under-performs our proposed method in all metrics.

%Finally, the results obtained for the GO-MPC-Off baseline show that for more than six agents, the learned guidance policy improves the collision avoidance performance in comparison with the pure MPC approach. Nevertheless, combining the MPC's collision avoidance performance with the guidance provided by the subgoal policy significantly improves the performance of our method.

\begin{table*}[!t]
 \caption{Statistics results for 200 runs of our proposed method (GO-MPC) comparing to the baselines: average time to goal and average traveling distance for the successful episodes, and number of episodes resulting in collision for $n \in \{6,8,10\}$ agents. For the mixed setting, we consider a distribution of 80\% cooperative and 20\% non-cooperative agents.}
        \centering
\begin{tabular}{|p{1cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|}
\hline
\multicolumn{2}{|c|}{} & \multicolumn{3}{c|}{Time to Goal [s]} & \multicolumn{3}{|c|}{\% failures (\% collisions / \% deadlocks) } & \multicolumn{3}{c|}{Traveled Distance Mean [m]} \\ \hline
\multicolumn{2}{|c|}{\# agents}                    & \multicolumn{1}{c|}{6}                & \multicolumn{1}{c|}{8}       & \multicolumn{1}{c|}{10}                        & \multicolumn{1}{c|}{6}                &\multicolumn{1}{c|}{8}     & \multicolumn{1}{c|}{10}                       & \multicolumn{1}{c|}{6}                & \multicolumn{1}{c|}{8}       &\multicolumn{1}{c|}{10}        \\ \hline \hline \multicolumn{11}{l}{\bf Mixed Agents} \\  \hline \hline
\multicolumn{2}{|c|}{MPC}                            & \multicolumn{1}{c|}{12.65}      &  \multicolumn{1}{c|}{15.88}          &     \multicolumn{1}{c|}{ 15.04}          & \multicolumn{1}{c|}{6 (5 / 1)}       & \multicolumn{1}{c|}{ 14 (8 / 6)}     &   \multicolumn{1}{c|}{18 (10 / 8) }            &  \multicolumn{1}{c|}{ 12.48}                &   \multicolumn{1}{c|}{13.05}       & \multicolumn{1}{c|}{13.13}   \\ \hline
\multicolumn{2}{|c|}{DRL~\cite{everett2019collision}}                      &  \multicolumn{1}{c|}{14.23}     &  \multicolumn{1}{c|}{15.13}       &    \multicolumn{1}{c|}{16.28 }         & \multicolumn{1}{c|}{ 17 (17 / 0)}    &  \multicolumn{1}{c|}{23 (23 / 0)}        &  \multicolumn{1}{c|}{29 (29 / 0)  }        &  \multicolumn{1}{c|}{13.75}   &   \multicolumn{1}{c|}{14.56}       & \multicolumn{1}{c|}{15.61}    \\ \hline
\multicolumn{2}{|c|}{DRL-2~\cite{everett2019collision}}                      &  \multicolumn{1}{c|}{14.03 }    & \multicolumn{1}{c|}{15.41 }        &    \multicolumn{1}{c|}{16.54}          & \multicolumn{1}{c|}{ 6 (6 / 0)}     & \multicolumn{1}{c|}{10 (10 / 0)}         &  \multicolumn{1}{c|}{13 (13 / 0)}           & \multicolumn{1}{c|}{13.92}    &  \multicolumn{1}{c|}{15.03}        & \multicolumn{1}{c|}{16.16}     \\ \hline
%\multicolumn{2}{|c|}{GO-MPC-Off}                &  \multicolumn{1}{c|}{14.58}               &  \multicolumn{1}{c|}{18.50 }            &  \multicolumn{1}{c|}{ 18.85}      & \multicolumn{1}{c|}{17 (17 / 0)}    &  \multicolumn{1}{c|}{19 (17 / 2)}          &  \multicolumn{1}{c|}{25 (22 / 3)}          & \multicolumn{1}{c|}{14.35}                & \multicolumn{1}{c|}{15.41}    &     \multicolumn{1}{c|}{16.14 }         \\ \hline
\multicolumn{2}{|c|}{GO-MPC}                &   \multicolumn{1}{c|}{13.85}              &   \multicolumn{1}{c|}{\textbf{14.48}}            &  \multicolumn{1}{c|}{\textbf{14.78}}       & \multicolumn{1}{c|}{\textbf{ 0 (0 / 0) }}    &  \multicolumn{1}{c|}{\textbf{ 0 (0 / 0)   }}        & \multicolumn{1}{c|}{\textbf{ 0 (0 / 0)   }}      & \multicolumn{1}{c|}{14.63}                &\multicolumn{1}{c|}{15.19 }    &      \multicolumn{1}{c|}{15.59}         \\ \hline \hline \multicolumn{11}{l}{\bf Homogeneous} \\  \hline \hline
\multicolumn{2}{|c|}{MPC}                &   \multicolumn{1}{c|}{17.37 }              &    \multicolumn{1}{c|}{16.38}          &  \multicolumn{1}{c|}{14.64}          &  \multicolumn{1}{c|}{ 30 (29 / 1)}     &  \multicolumn{1}{c|}{36 (25 / 11)}          &   \multicolumn{1}{c|}{ 35 (28 / 7)}              & \multicolumn{1}{c|}{ 11.34}      & \multicolumn{1}{c|}{10.86 }    & \multicolumn{1}{c|}{10.62}        \\ \hline
\multicolumn{2}{|c|}{DRL~\cite{everett2019collision}}                &  \multicolumn{1}{c|}{ 14.18}           &     \multicolumn{1}{c|}{14.40}                   &    \multicolumn{1}{c|}{14.64 }                &   \multicolumn{1}{c|}{16 (14 / 2) }               &   \multicolumn{1}{c|}{20 (18 / 2)}                  & \multicolumn{1}{c|}{20 (20 / 0) }      &   \multicolumn{1}{c|}{12.81}               &   \multicolumn{1}{c|}{12.23}               &    \multicolumn{1}{c|}{12.23}          \\ \hline
\multicolumn{2}{|c|}{DRL-2~\cite{everett2019collision}}                &  \multicolumn{1}{c|}{ 15.96}           &     \multicolumn{1}{c|}{17.47}                   &   \multicolumn{1}{c|}{15.96}                   &  \multicolumn{1}{c|}{17 (11 / 6)}                 &    \multicolumn{1}{c|}{ 29 (21 / 8)}                & \multicolumn{1}{c|}{28 (24 / 4)}       &   \multicolumn{1}{c|}{15.17 }              &   \multicolumn{1}{c|}{15.85}               &     \multicolumn{1}{c|}{15.40}       \\ \hline
%\multicolumn{2}{|c|}{GO-MPC-Off}                &  \multicolumn{1}{c|}{14.08}                   &    \multicolumn{1}{c|}{15.54}                    &    \multicolumn{1}{c|}{15.89}                 &   \multicolumn{1}{c|}{19 (17 / 2) }             &    \multicolumn{1}{c|}{29 (29 / 0)}            &   \multicolumn{1}{c|}{26 (26 / 0)}          &   \multicolumn{1}{c|}{14.25}           &  \multicolumn{1}{c|}{15.45}          & \multicolumn{1}{c|}{15.94}      \\
\hline
\multicolumn{2}{|c|}{GO-MPC}                &   \multicolumn{1}{c|}{\textbf{13.77}}         &    \multicolumn{1}{c|}{\textbf{14.30}}         &    \multicolumn{1}{c|}{\textbf{14.63}}         &  \multicolumn{1}{c|}{\textbf{  0 (0 / 0)  }} &  \multicolumn{1}{c|}{\textbf{  0 (0 / 0)  } }    &   \multicolumn{1}{c|}{ \textbf{ 2 (1 / 1)    }}   &    \multicolumn{1}{c|}{14.67}         &  \multicolumn{1}{c|}{15.09}         & \multicolumn{1}{c|}{15.12}      \\
\hline
\end{tabular}
 \label{tab:global_performance}
\end{table*}

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{images/collision_avoidance_comparison.png}
%    \caption{Collision avoidance performance of our proposed method vs two state-of-the-art baselines: GA3C \cite{everett2018motion} and CADRL \cite{chen2017socially}}
%    \label{fig:comparison_baselines}
%\end{figure}


